Quantifying identifiability to choose and audit $\epsilon$ in differentially private deep learning

Differential privacy allows bounding the influence that training data records have on a machine learning model. To use differential privacy in machine learning, data scientists must choose privacy parameters $(\epsilon,\delta)$. Choosing meaningful privacy parameters is key, since models trained with weak privacy parameters might result in excessive privacy leakage, while strong privacy parameters might overly degrade model utility. However, privacy parameter values are difficult to choose for two main reasons. First, the theoretical upper bound on privacy loss $(\epsilon,\delta)$ might be loose, depending on the chosen sensitivity and data distribution of practical datasets. Second, legal requirements and societal norms for anonymization often refer to individual identifiability, to which $(\epsilon,\delta)$ are only indirectly related. We transform $(\epsilon,\delta)$ to a bound on the Bayesian posterior belief of the adversary assumed by differential privacy concerning the presence of any record in the training dataset. The bound holds for multidimensional queries under composition, and we show that it can be tight in practice. Furthermore, we derive an identifiability bound, which relates the adversary assumed in differential privacy to previous work on membership inference adversaries. We formulate an implementation of this differential privacy adversary that allows data scientists to audit model training and compute empirical identifiability scores and empirical $(\epsilon,\delta)$.

==> defi.tex <==
%%custom packages
% Magic hack for subcaption and svg compatibility
% https://tex.stackexchange.com/questions/291929/svg-package-and-subcaption-incompability
\RequirePackage{scrlfile}
\PreventPackageFromLoading{subfig}

\usepackage[inline]{enumitem}
\usepackage{comment}
%\usepackage{cite}
\usepackage{todonotes}
\usepackage{csquotes}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{multicol} 
%\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{hyperref}
%\let\proof\relax
%\let\endproof\relax
%\usepackage{amsthm}
\usepackage{tikz}
\usepackage{pdfpages}
\usepackage{tabularx}
\usepackage{mathrsfs}
\usepackage{amsmath,amstext}
%\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage[thinc]{esdiff}
\usepackage{xspace}
\usepackage{adjustbox}

\usepackage{balance}
\usepackage{microtype}
\usepackage{cryptocode}
\usepackage{makecell}


\usetikzlibrary{shapes, fit}

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}

\usepackage{url}
\usepackage{textcomp}
\usepackage{color}
\graphicspath{{figures/}}
%% Custom definitions
\newcommand{\eps}{\ensuremath{\epsilon}\xspace}
\newcommand{\feps}{\ensuremath{\epsilon'}\xspace}

\newcommand{\dlt}{\ensuremath{\delta}\xspace}
\newcommand{\sgm}{\ensuremath{\sigma}\xspace}
\newcommand{\tht}{\ensuremath{\theta}\xspace}
\newcommand{\epsdlt}{\ensuremath{(\epsilon,\delta)}\xspace}
\newcommand{\money}[1]{\$#1}
\newcommand{\person}[1]{\textsc{#1}}
\newcommand{\cali}[1]{\ensuremath{\mathcal{#1}}} % for uppercase letters only
\newcommand{\var}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\varbf}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\subscr}[2]{\ensuremath{#1_{\var{#2}}}}
\newcommand{\supscr}[2]{\ensuremath{#1^{\var{#2}}}}
\newcommand{\subsup}[3]{\ensuremath{#1_{\var{#2}}^{\var{#3}}}}
\newcommand{\pprime}{\ensuremath{\prime}}
\newcommand{\filenamename}{\edef\foo{\currfilebase}}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\Z}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\R}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\N}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}\xspace}

\newcommand{\Ami}{\mathcal{A}_{\var{MI}}}
\newcommand{\Astrong}{\mathcal{A}_{\var{DI}}}
\newcommand{\AstrongGau}{\mathcal{A}_{\var{DI, Gau}}}

\newcommand{\datapoint}{x}

\newcommand{\madi}{\mathrm{Adv}^{\mathrm{DI}}}
\newcommand{\madiGau}{\mathrm{Adv}^{\mathrm{DI, Gau}}}
\newcommand{\mami}{\mathrm{Adv}^{\mathrm{MI}}}

\newcommand{\edi}{\mathrm{Exp}^{\mathrm{DI}}}
\newcommand{\emi}{\mathrm{Exp}^{\mathrm{MI}}}

\newcommand{\ra}{\mathrm{\rho}_{\mathrm{\alpha}}}
\newcommand{\rb}{\mathrm{\rho}_{\mathrm{\beta}}}

\newcommand{\dpgrad}{\ensuremath{\tilde g}\xspace}
%clippedgrad
\newcommand{\clgrad}{\ensuremath{\hat{g}}\xspace}

\newcommand{\sens}{\ensuremath{\Delta f}\xspace}

\newcommand{\clip}{\ensuremath{\var{C}}\xspace}

% uncomment for IEEE / comment for ACM
%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
%\newtheorem{definition}{Definition}

%\newtheoremstyle{defistyle}% name für den Stil
%
%  {}%      Space above
%
%  {}%      Space below
%
%  {\itshape}%      Body font
%
%  {}%      Indent amount (empty = no indent, \parindent = para indent)
%
%  {\bfseries\sffamily}% Thm head font
%
%  {\rm.}%        Punctuation after thm head
%
%  { }% Space after thm head: " " = normal interword space; \newline = linebreak
%
%  {} %{\textbf{\thmname{Definition}} (\thmnote{#3})}%         Thm head spec (can be left empty, meaning `normal')
%
%  % http://www.stat.umn.edu/~charlie/amslatex.html <http://www.stat.umn.edu/~charlie/amslatex.html> 
%
%\theoremstyle{defistyle}

% quotes

\newcommand{\bq}{``}

\newcommand{\red}[1]{\textcolor{black}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\revised}[1]{\textcolor{blue}{#1}}

\newcommand{\eq}{''}

\newcommand{\q}[1]{\bq{#1}\eq}

\renewcommand{\vec}[1]{\mathbf{#1}}

\newcommand{\Rkk}{R_{k}}

\let\oldReturn\Return
\renewcommand{\Return}{\State\oldReturn}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{experiment}{Experiment}
\newtheorem{proposition}{Proposition}

\newif\iffullversion
\fullversiontrue

==> src/application_synth.tex <==
\section{Validation over synthetic data}
\label{sec:val}

In this section we demonstrate how the confidence and membership advantage of $\cali{A}_{\var{adapt}}$ develop in an empirical example. We evaluate how well $\rho_c$ and $\rho_a$ actually model the true risk for data members and how effective $\cali{A}_{\var{adapt}}$ behaves on synthetic data. As $\cali{A}_{\var{adapt}}$ is assumed to know all data member except for one, the size of $\cali{D}$ does not influence her. For this reason, we consider the following tiny data universe $\cali{U}$, true data set $\cali{D}$ and alternative $\cali{D'}$ presented in Tables~\ref{tab:data-universe}, \ref{tab:data-set} and \ref{tab:prior-knowledge}. Let $\cali{U}$ represent a set of employees that were offered to participate in a survey about their hourly wage. Alice, Bob and Carol participated. Dan did not. Thus, the survey data $\cali{D}$ consists of 3 entries. The survey owner allows data analysts to pose queries to $\cali{D}$ until a DP budget (see \cite{McSherry2009}) of ($\eps=5$, $\dlt=0.01$) is consumed. $\cali{A}_{\var{adapt}}$ is the data analyst that queries $\cali{D}$. Aside from learning statistics about the wage, $\cali{A}_{\var{adapt}}$ is also interested in knowing about who participated. So far, she knows that Alice and Carol participated for sure and there are three people in total. Thus, she has to decide between $\cali{D}$ and $\cali{D'}$, i.e., whether Bob or Dan is the missing entry. As a side information, she knows that the employer pays at least \$1 and a maximum of \$10. As a consequence, when we let $\cali{A}_{\var{adapt}}$ ask only the sum query function, $\cali{S}(f)=\Delta f_2=9$. Further, the Gaussian mechanism is known to be used for anonymization.  

\begin{table}[tp]
	\centering
	\begin{minipage}[b]{.32\linewidth}
		\centering
		\begin{tabular}{|ll|}
			\hline Name & Wage \\
			\hline Alice & \$5 \\
			Bob & \$10 \\
			Carol & \$2 \\
			Dan &  \$1\\
			\hline
		\end{tabular}
		\caption{$\cali{U}$}
		\label{tab:data-universe}
	\end{minipage}\hfill
	\begin{minipage}[b]{.32\linewidth}
		\centering
		\begin{tabular}{|ll|}
			\hline Name & Wage \\
			\hline Alice & \$5 \\
			Bob & \$10 \\
			Carol & \$2 \\
			\hline
		\end{tabular}
		\caption{$\cali{D}$}
		\label{tab:data-set}
	\end{minipage}\hfill
	\begin{minipage}[b]{.32\linewidth}
		\centering
		\begin{tabular}{|ll|}
			\hline Name & Wage \\
			\hline Alice & \$5 \\
			Dan &  \$1\\
			Carol & \$2 \\
			\hline
		\end{tabular}
		\caption{$\tilde{\cali{D}}$}
		\label{tab:prior-knowledge}
	\end{minipage}
\end{table}

Given these prior information, $\cali{A}_{\var{adapt}}$ iteratively updates her belief on $\cali{D}, \cali{D'}$ after each query. She makes a final guess after the whole \epsdlt-budget has been used. By using our proposed framework ($\rho_c, \rho_a$), all data members (especially Bob in this case) can compute their protection guarantee: What is the advantage of $\cali{A}_{\var{adapt}}$ in disclosing a person's participation (i.e., $\rho_a$)? How plausibly can that person deny a revelation (i.e., $\rho_c$) by $\cali{A}_{\var{adapt}}$? Referring to Definition~\ref{def:expected-adversarial-success-rate} and Definition~\ref{def:general-upper-bound}, we compute $\rho_a(5,0.01) = 0.5$ under composition and $\rho_c(5,0.01) = 0.99$ illustrating that the risk of re-identification is quite high and the deniability extremely low.
However, to show if $\cali{A}_{\var{adapt}}$ actually reaches those values we empirically analyze her behavior by iteratively querying $\cali{D}$ and applying Algorithm~\ref{alg:adaptive-attacker} after each query. We use $k=100$ queries and repeat the experiment 10000 times to estimate membership advantage and show the distribution of confidence at the end of each run. As we know that the adversary will compose $k$ times, we use the RDP composition scheme to determine what noise scale must be applied for each individual query. In Figure~\ref{fig:synthethic-attack-sample} the adaptive posterior beliefs for $\cali{D}$ and $\cali{D'}$ are depicted. After some fluctuation, the belief for $\cali{D}$ starts growing up to $0.90$. Consequently, the final guess of $\cali{A}_{\var{adapt}}$ is $\cali{D}$ which is correct. The guesses over all runs are summarized in Figure~\ref{fig:synthethic-attack-guesses}. Here, we see that about 75\% of the guesses of $\cali{A}_{\var{adapt}}$ are correct which corresponds exactly to the expected membership advantage of our threat model. However, the predicted upper bound of $0.99$ was not reached in the sample run. In contrast to $\rho_a$, $\rho_c$ is a worst case bound, not an expectation. Thus, the final belief of $\cali{A}_{\var{adapt}}$ approaches $\rho_c$ very rarely.  

\begin{figure}
	\centering    
	\begin{subfigure}[b]{0.64\linewidth}     
		\includegraphics[width=\linewidth]{figures/synthethic_attack_sample.pdf}      
		\subcaption{Sample run}
		\label{fig:synthethic-attack-sample}      
	\end{subfigure}     
	\begin{subfigure}[b]{0.34\linewidth} 
		\includegraphics[width=\linewidth]{figures/synthethic_guesses_sample.pdf}      
		\subcaption{Guesses}
		\label{fig:synthethic-attack-guesses}
	\end{subfigure}
	\caption{(a) Sample run of $\cali{A}_{\var{adapt}}$ on a sequence of $k=100$ evaluations of $\cali{M}_{Gau_i}$ that shows the mechanism outputs on the left y-axis and the development of posterior belief for $\cali{D}$ and $\cali{D}'$ on the right-hand y-axis. At the end of each sample run $\cali{A}_{\var{adapt}}$ decides for the data set with the highest posterior belief. In (b), the number of decisions for over all runs are shown.}
	\label{fig:synthetic-experiment}
\end{figure}

To illustrate this phenomenon, we plot a histogram over the beliefs at the end of each run for various choices of $\rho_c$ in Figure~\ref{fig:belief-distribution}. We see that the predicted worst case bound was reached in a small proportion of runs. This effect becomes more visible when $\eps$ is lower.

A final note on $\dlt$ which describes the probability of exceeding $\rho_c$. When looking closely at the histograms, one can see that there are some (small) columns for a range of values that are larger than the worst-case bound. We calculate their proportion to all runs, e.g., $0.0008$ for $\eps=5$ which is close to the promised error.

\begin{figure*}
	\centering    
	\begin{subfigure}[b]{0.24\linewidth}     
		\includegraphics[width=\linewidth]{figures/synthethic_attack_belief_distributions_rho75.pdf}      
		\subcaption{$\eps=1.10, \rho_c(1.10,0.01)=0.75$}
		\label{fig:belief-dist-eps1}      
	\end{subfigure}%
    \hfill  
	\begin{subfigure}[b]{0.24\linewidth} 
		\includegraphics[width=\linewidth]{figures/synthethic_attack_belief_distributions_rho90.pdf}      
		\subcaption{$\eps=2.20, \rho_c(2.20,0.01)=0.90$}
		\label{fig:belief-dist-eps3}
	\end{subfigure}%
	\hfill  
	\begin{subfigure}[b]{0.24\linewidth} 
		\includegraphics[width=\linewidth]{figures/synthethic_attack_belief_distributions_rho95.pdf}      
		\subcaption{$\eps=2.94, \rho_c(2.94,0.01)=0.95$}
		\label{fig:belief-dist-eps5}
	\end{subfigure}%
	\hfill  
	\begin{subfigure}[b]{0.24\linewidth} 
		\includegraphics[width=\linewidth]{figures/synthethic_attack_belief_distributions_rho99.pdf}      
		\subcaption{$\eps=4.60, \rho_c(4.60,0.01)=0.99$}
		\label{fig:belief-dist-eps10}
	\end{subfigure}
	\caption{Confidence distribution of $\cali{A}_{\var{adapt}}$ at the end of all $10,000$ runs, i.e., after composition. We show this distribution over different $\eps$ and fixed $\dlt=0.001$. As expected in some cases at the tails of the histogram  the respective noise upper bound is reached.}
	\label{fig:belief-distribution}
\end{figure*}
